RP2K: A Large-Scale Retail Product Dataset for Fine-Grained Image Classification

We introduce RP2K, a new large-scale retail product dataset for fine-grained image classification. Unlike previous datasets focusing on relatively few products, we collect more than 500,000 images of retail products on shelves belonging to 2000 different products. Our dataset aims to advance the research in retail object recognition, which has massive applications such as automatic shelf auditing and image-based product information retrieval. Our dataset enjoys following properties: (1) It is by far the largest scale dataset in terms of product categories. (2) All images are captured manually in physical retail stores with natural lightings, matching the scenario of real applications. (3) We provide rich annotations to each object, including the sizes, shapes and flavors/scents. We believe our dataset could benefit both computer vision research and retail industry. Our dataset is publicly available at https://www.pinlandata.com/rp2k_dataset.

==> app.tex <==

\appendix
% \section{Statement of Broader Impact}\label{sec:broader}
% A robust retail object recognition system is desired in a myriad of applications in AI-powered retail store.
% It is foreseeable that our dataset can be served as a starting point for any retail applications using shelf images.
% Future applications based on retail object recognition system include but not limit to:

% \paragraph{Auditing product placement.}
% Auditing shelf management using object recognition system digitizes store plays an essential role in understanding the shelf conditions.
% On the one hand, costumers may mistakenly place products they don't want to buy on the wrong shelf.
% Identifying the wrong placement requires a lot of human resources in traditional retail store, but it can be immediately detected by computer system.
% On the other hand, some analysis show that customer make important buying decisions based on the placement of store shelves,
% and retailers invest to create ideal planograms as their selling strategy. It is crucial that to make sure the products are placed in their desired way.

% \paragraph{Detecting empty shelf.}
% Empty shelf is an indicator of whether a product is out-of-stock. In many cases, the retailers have more available stocks in their warehouse even their store shelves show out-of-stock. 
% Before the retailer refill the stocks, it even takes a certain amount of time for the retailer to realize the product is out-of-stock.
% With a robust recognition deployed in the store, the store can quickly send notification of which product is out-of-stock and tracking the selling activities in real-time.

% % \paragraph{Assessing competition.}
% \paragraph{Image-based product retrieval.}
% Not only for the retailer, the costumer could also benefit from a well-established in-store object recognition system.
% Imagine you want to search information for a particular product in-store, instead of Googling the product name on web,
% you can take a photo of the product and the information will immediately prompt out.
% Moreover, based on the image, your location information could also be retrieved, rendering a image-based navigation system.
% This could increase the accessibility of the retail store.

%=========================================

% High-quality speech denoising is desired in a myriad of applications: human-robot interaction, cellular
% 308 communications, hearing aids, teleconferencing, music recording, filmmaking, news reporting, and
% 309 surveillance systems to name a few. Therefore, we expect our proposed denoising method—be it a
% 310 system used in practice or a foundation for future technology—to find impact in these applications.

% \paragraph{Auditing product placement.}
% Customers make important buying decisions at store shelves. Companies invest in tools and studies to create planograms that are part of their ideal store strategy. Auditing shelf management using Image Recognition digitizes store checks and plays an essential role in understanding the shelf conditions and how they affect the sales of their core SKUs.
% Object Detection, using a deep neural network, detects SKUs within images of shelves and classifies them at manufacturer, brand or SKU level. Such a neural network can be trained to compare and identify gaps between actual shelf image and reference planogram. Depending upon the accuracy and speed of these neural networks, the auditor can get real-time feedback on their handheld device to take corrective actions while they are still in store.
% Leveraging object detection in retail can make store checks productive and empower your sales rep or auditor to take corrective actions and fix issues.

% \paragraph{Detecting empty shelf.}
% A study conducted by IHL group puts the total loss of sales due to out of stock at nearly \$1 trillion. The study found that over 20\% of Amazon’s North American Retail revenue can be attributed to consumers who first tried to buy the product at a local store but found it out-of-stock.
% Empty shelves were encountered by 32\% of the shoppers in the study and thus, retailers and CPG firms need to ensure the shelf are always stocked with the correct product. Retailers can leverage Image Recognition and Object Detection using fixed cameras in their store to alert the store staff whenever a shelf is found to be empty. The store staff can get an instant alert on their phone along with the accurate description of the SKU missing from the shelf and the location of the shelf.

% \paragraph{Assessing competition}
% Object Detection algorithms can also be trained to identify competitive activity in-store and spot category trends.
% While retail data provide information on category sales for different brands, it does not accurately capture the in-store activities of different brands that drive sales.
% Identifying competitor and tracking their in-store activity can help a brand to grow in their category by identifying potential opportunities. A large tobacco company was able to track the new launches of its competitors and their promotional programs using Image Recognition provided by ShelfWatch. They were able to cross-reference new launches and in-store promotions of their competitors with the retail sales data to identify new areas of growth.


\newpage
\section{Additional Samples of Shelf Images} \label{sec:shelf}

% \begin{figure}[h]
%   \centering
% %   \vspace{-2mm}
%     \includegraphics[width=0.5\columnwidth]{figs/shelf/1.jpg}
%     % \vspace{-2.9mm}
%     % \caption{Sample images from our dataset with different meta-categorizations. \textbf{(top)} Categorized by product types. 
%     % \textbf{(bottom)} Categorized by product shapes.
  
% %   \vspace{-3.8mm}
% \end{figure}

\begin{figure}[h]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{figs/shelf/beer1.jpg}
    \caption{Beer.}

\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{figs/shelf/seasoning1.jpg}
    \caption{Seasoning.}

\end{subfigure}

\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{figs/shelf/cosmetics2.jpg}
    \caption{Cosmetics.}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{figs/shelf/liquor1.jpg}
    \caption{Liquor.}

\end{subfigure}


\caption{Additional shelf images.}
\end{figure}


\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{figs/shelf/diary1.jpg}
    \caption{Dairy.}

\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{figs/shelf/seasoning3.jpg}
    \caption{Seasoning.}

\end{subfigure}

\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{figs/shelf/drink1.jpg}
    \caption{Non-Alcoholic Drink.}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{figs/shelf/cosmetics3.jpg}
    \caption{Cosmetics.}

\end{subfigure}


\caption{More additional shelf images.}
\end{figure}


\newpage

\section{Additional Samples of Object Images} \label{sec:obj}

\begin{figure}[h]
  \centering
%   \vspace{-2mm}
    \includegraphics[width=1.0\columnwidth]{figs/moresamples1.pdf}
    % \vspace{-2.9mm}
    \caption{Additional images with different SKUs.}
    % \textbf{(bottom)} Categorized by product shapes.
  
%   \vspace{-3.8mm}
\end{figure}

\begin{figure}[h]
  \centering
%   \vspace{-2mm}
    \includegraphics[width=1.0\columnwidth]{figs/moresamples2.pdf}
    % \vspace{-2.9mm}
    \caption{More images with different SKUs.}
    % \textbf{(bottom)} Categorized by product shapes.
  
%   \vspace{-3.8mm}
\end{figure}

\newpage


\section{Auxiliary Detection Dataset} \label{sec:detection}
% Since classifying products accurately requires a robust detection algorithm that can extract the bounding box of the product, it is important to understand how well the standard detection pipeline would work on our dataset.
% Thus, we also provide a auxiliary object detection dataset to evaluate detection algorithm on our dataset.
% It is worth noting that detecting bounding boxes of shelf objects and be treated as another separate problem, and there exist many solutions on this problem~\cite{goldman2019precise,hao2019take}.
% We collect in total \ref{X} bounding boxes, based on the shape classification described in \secref{obj}:
Here we provide the evaluation on the auxiliary detection dataset.
We split the 95,800 bounding boxes to 80,000 training boxes and 15,800 test boxes.
We use the standard RetinaNet~\cite{lin2017focal} to evaluate the detection performance.
We report the Average Precision (AP) for each shape, as well as mean Average Precision (mAP) for the entire test set, with different IoU threshold, the results are summarized in \tabref{detection}.

% In this section we provide our experiment on the object detection task of our dataset.


% \subsection{Product Detection}
% Since classifying products accurately requires a robust detection algorithm that can extract the bounding box of the product, it is important to understand how well the standard detection pipeline would work on our dataset.
% In this section we provide our experiment on the object detection task of our dataset.

% The detailed performance can be found in \tabref{detection}.
\begin{table}[h]
  \caption{Performance of object detection. AP($x$) indicates AP with IoU threshold=$x$.}
  \label{tab:detection}
  \centering
%   \resizebox{1.0\textwidth}{!}{% <------ Don't forget this %

\begin{tabular}{l|cccccccc}
\bottomrule
Shape & AP(0.5) & AP(0.55) & AP(0.6) & AP(0.65) & AP(0.7) & AP(0.75) & AP(0.8) \\ \hline
Box &  0.3485&  0.3475 &   0.344    & 0.3372 & 0.3195 &  0.3003 & 0.2670          \\
Can &   0.6886& 0.6868 &    0.6837  & 0.6811& 0.6766  &  0.6650 & 0.6314\\
Bottle & 0.7525& 0.7509 &   0.7487  & 0.7448& 0.7365  &  0.7137 & 0.6545\\
Jar &   0.2620&  0.2559 &   0.235   & 0.2302& 0.2191  &  0.1921 & 0.1748  \\
Handled Bottle & 0.4919& 0.4896  &  0.4658 & 0.4505 & 0.4014 & 0.3804 & 0.3059\\
Bag & 0.3449 &  0.338 & 0.3273 & 0.3151& 0.2827 & 0.2518 & 0.1901          \\
Pack & 0.4643 & 0.4634 & 0.4634 & 0.4634&  0.4634 & 0.4494 & 0.3789\\ \hline
mAP for All & 0.6186&  0.6164 & 0.6121 & 0.6069  & 0.5962 & 0.5739 & 0.3994 \\
% Class & Box(S) & Box(L)  & Jar & Bottle & Can & Bag & Bucket & Others\\ \hline
% \#Instances & 1107 & 280 & 260 & 1914 & 7445 & 1120 & 590 & 4023 \\
% AP & 0.4159 &0.7418 & 0.4147 & 0.7972 & 0.7637 & 0.4026 & 0.4830 & 0.2076 \\
% Class & Bottle & Can & Box & Bag & Jar & Handled Bottle & Pack \\ \hline
% \# Instances & 48,958 & 14,320 &7,167 & 7,943 & 3,769 & 3,682 & 9,964 \\
% AP & 0.7525 & 0.6886 & 0.5504 & 0.3449 & 0.262 & 0.4919 & 0.6223 \\

 \toprule
\end{tabular}
% }
\end{table}

% \begin{table*}[h]
% \centering
% % \resizebox{.5\textwidth}{!}{
% % \hspace{-7mm}
% \begin{tabular}{l|cccccccc}
% \bottomrule
%  & \multicolumn{7}{c}{Models}\\
%              & Untrained  & 1 epoch  & 2 epochs & 5 epochs & 10 epochs& 15 epochs & 20 epochs & Adv. trained \\ \hline
% Standard Acc. &   81.8\%  &  81.6\%  & 82.4\%   & 83.0\%   &  82.4\% &  82.2\% & 82.7\%    &  82.9\%   \\
% BPDA-I Acc.&      30.6\%  &  30.7\%  & 40.0\%   & 46.4\%   &  62.3\%  & 63.1\%& 62.9\%    &  80.5\%        \\
% Avg. $\ell_{\infty}$&     0.005   &   0.033  &  0.036     & 0.067     &  0.130    & 0.133& 0.136      &  0.272      \\
% \toprule
% \end{tabular}
% % }
% \caption{Relationship between expected adversarial image and test accuracy under BPDA-I. We use perturbation size $\epsilon=0.2$ here.}\label{tab:expected_img}
% \end{table*}

% \section{Discussion on Performance}

